Evaluating Nonlinear Decision Trees for Binary Classification Tasks with Other Existing Methods

Classification of datasets into two or more distinct classes is an important machine learning task. Many methods are able to classify binary classification tasks with a very high accuracy on test data, but cannot provide any easily interpretable explanation for users to have a deeper understanding of reasons for the split of data into two classes. In this paper, we highlight and evaluate a recently proposed nonlinear decision tree approach with a number of commonly used classification methods on a number of datasets involving a few to a large number of features. The study reveals key issues such as effect of classification on the method's parameter values, complexity of the classifier versus achieved accuracy, and interpretability of resulting classifiers.

==> GAMs_Sparsh.tex <==
\subsection{Generalized Additive Method (GAM)}

The Generalized Additive Models (GAMs)\cite{wood2017generalized} are the machine learning models which are of the expression:
\begin{equation*}
    M(E[y|X]) = \beta_0 + f_1(x_1) + f_2(x_2) + ... + f_k(x_n,x_m) +...+f_m(x_n)
\end{equation*}

where the 
\textcolor{blue}{$ [x_1, x_2, ..., x_N]$}
are independent variables or the attributes of the Dataset, $ \textcolor{red}{y} $ is the dependent variable on the independent ones, and $M$ is the function that relates our predictor variables to the anticipated values of the y variable.\\

The functions $f_i()$ are accomplishment of the combination of Splines, which are combined weighted with their respective coefficients.


\subsubsection*{What are Splines?}
\Sparsh{\Yashesh{} Can you Remove the colon just-before}\\
The Splines\cite{eilers1996flexible} are piece-wise Polynomials over a specific intervals used for mainly 2 purposes that is:- Interpolation and Smoothing tasks.\\ The Splines can be fitted over any $n-dimensional$ dataset.\\
A general representation of the Splines is as follows:-

\[ S(x) \textbf{=} \begin{cases} 
          S_1(x) &  x_0\leq x\leq x_0 \\
          S_2(x) & x_1\leq x\leq x_2 \\
          ...\\
          S_{n-1} & x_{n-1}\leq x \leq x_n
       \end{cases}
    \]

where the $S_i(x) $ is a polynomial of some degree fitted over datapoints in that particular interval. 


The Linear Models of Machine Learning can be thought of as a subset of GAMs or like a special case of GAMs.\\
\begin{figure}[hbtp]
    \centering
    \includegraphics[width = 0.5\linewidth]{All_plots/gam_lm.PNG}
    \caption{(Generalized Additive Model) GAM and (Linear Model) LM}
    \label{fig:Gam subset of lm}
\end{figure}

So to recap, in the Linear Models\cite{bishop2006pattern} a single coefficient is fitted with respect to a single feature vector. So, at the end we have like a single line associated with one feature, then all such \quotes{lines} have been summed-up together in a Linear model. Eg- Least Squares is a familiar example of a Linear Model in Machine Learning\cite{bishop2006pattern}.

%%%%%%%%%%%%%%%% Shift this image to right %%%%%%%%%%%%%%

\begin{figure}[hbtp]
    \centering
    \includegraphics[width = \linewidth]{Pictures(NotPlots)/LinearModelRepresentation.png}
    \caption{LINEAR MODEL.
    In it 1 Coefficient is fitted per feature vector. Hence, at the end we have 1 line per feature vector, \& we can \quotes{sum} those lines together to make a prediction.}
\end{figure}

The GAMs are also pretty much similar to the LMs as shown before but here instead of a line, we fit a possibly non-linear function.

%Correct this ASAP, text not appearing

\begin{figure}[hbtp]
    \centering
    \includegraphics[width = \linewidth]{figures/illustrations/GamRepresentation.png}
    \caption{GAM for a simple regression case. Here we can see that it is very much akin to the Linear Model where we had 1 coefficient per feature vector, but here we can have a Non-linear function.}
\end{figure}

\subsubsection*{What are GAMs?\\}

To put it simply the GAMs are the extension of (Generalized Linear Models) GLMs  when combined with Splines and a Smoothing Penalty.

%\clearpage

\begin{figure}[hbtp]
    \centering
    \includegraphics[width = \linewidth]{Pictures(NotPlots)/GamBreakDown.png}
    \caption{DISMANTLED ASSESSMENT OF THE GAMs. The GAMs can be perceived as a combination of the GLMs (Generalized Linear Models), Weighted Splines \& Smoothing Penalty applied on the used Splines to control wiggliness}.
\end{figure}

GAMs extend the generalized linear models by allowing non-linear functions of the features whilst maintaining the additivity, this \quotes{additivity} nature carries forward the Interpretability part of the Linear Models. As the GAMs are additive, it is very much easy to examine the effect of each $x_i$ on Y individually while holding all other predictors constant.\\
Hence, the result is a very flexible model, where it is very easy to incorporate prior knowledge and control overfitting.

\subsubsection{\textbf{Work Flow [Overview of the Experimental Set-up]}\\}

Let's say for a Dataset with n-features. We have to apply GAMs on it, to build a classifier.\\
Here we will be splitting the Raw Data in $train$ \& $test$, with $test\_data$ size being 30\% of the Raw Data.\\
We will be using $LogisticGAM$ for binary classifiers to be built.
So, for each of the attribute we will be using $s()$ ie- Spline as functional-form term.
For each of the Spline Term associated with a single attribute,we mainly would be varying $n\_splines$ (number of the Splines affiliated to the respective attribute) \& $ spline\_order $ (order of the Splines affiliated to the respective attribute). And rest of the hyperparameters are kept at their default values.

\noindent Now arbitrarily \quotes{varying} the 2 hitherto hyperparameters is going to very much computationally expensive therefore, we devised some range of values from which their value will be randomly chosen from:-
$
\\
\textbf{n\_splines} := [ 2, 3, 5, 8, 13, 21]\\
\textbf{spline\_order} := [ 2,3,5 ]
$

Number\_of\_parameter \& Rule length was also calculated for all the models, and their \textbf{mean $\pm$ std.} was reported.

For example:- for a Dataset with \textbf{\textit{n}} attributes, \& a PyGam Model is fitted with $s()$ as the model function for the n-features. Then in that case the \textbf{Interpretability} judging values are calculated as follows:-

RuleLength = \\$ \sum_{i=1}^{i=n} {(order\_splines(i) + 1)*n\_splines(i) + n\_splines(i) + 1 }$
\\

\#Parameters = $ \sum_{i=1}^{i=n} {n\_splines(i)*order\_splines(i)} + 1
$

%mention




\subsubsection{Results}
The Results for GAM are generated and analysed for various Datasets.

\begin{table*}[ht]
    \centering
    \caption{Results Achieved on Various Datasets by GAM}
    \label{tab:gam_results}
    \begin{tabular}{|c|c|c|c|c|}
    \hline
    \textbf{Sr. No.} & \textbf{Dataset} & \textbf{Rule Length} & \textbf{Number of Parameter} & \textbf{Accuracy}\\
    \hline
    1    &   DS1    &    122.285$\pm$ 53.437 &    75.287 $\pm$ 38.233 & 100.0 $\pm$ 0.0                       \\
    \hline
    2     & DS2 & 123.373 $\pm$ 54.324 & 76.124 $\pm$ 39.223 & 100.0 $\pm$ 0.0\\
    \hline
    3 & DS3 & 123.127 $\pm$ 52.285 & 75.912 $\pm$ 37.714 & 99.989 $\pm$ 0.134 \\
    \hline
    4 & DS4 & 122.384 $\pm$ 55.213 & 75.47 $\pm$ 39.375 & 47.143 $\pm$ 4.631 \\
    \hline
    5 & Truss Dataset &   186.922 $\pm$ 64.938 & 114.72 $\pm$ 46.674 & 95.246 $\pm$ 1.846                                  \\
    \hline
    6 & Welded Beam Dataset  & 245.132 $\pm$ 75.342  & 149.671 $\pm$ 53.982 & 99.710 $\pm$ 0.352 \\
    \hline
    7 & dtlz1\_3\_30 & 1856.329 $\pm$ 207.203 & 1130.247 $\pm$ 147.975 & 52.0329 $\pm$ 0.756 \\
    \hline
    8 & Cancer(10F) & 555.68 $\pm$ 132.63 & 339.45 $\pm$ 92.206 & 95.10 $\pm$ 0.713 \\
    \hline
    
    \end{tabular}
\end{table*}



Here the Number of Parameters is defined by taking those parameters which are "learned" from the data instead of the Hyperparameters (which are set manually example:- lambda).
For eg- In a ANN the number of weights will account for the number of parameters. But epochs, number of layers will not be accounted for.\\

Our Results on the Datasets:-\\
We will discuss plot:- Number of Parameters vs Error.

% This figure is for Truss data Set

% \begin{figure}
% \includegraphics[width = 150 mm, scale= 0.7]{figures/Plot_truss.jpeg}
% \caption{Put Error in Log Scale. See also how the plot looks if you put X-axis also in the log scale. We go }
% \end{figure}






\noindent {\bf Advantages:} If a downloadable code is available, mention it here.
\begin{itemize}
    \item It's syntax is very much straight-forward, and is very much similar to Sklearn (another Machine Learning Package)\cite{scikit-learn}. Due to their simple syntax they can be used straight out of the box.
    
    \item Inbuilt Result Visualization Functions to generate plots like Partial Dependence plots.
    
    
    
\end{itemize}

\noindent {\bf Disadvantages:}

\begin{itemize}
    \item Though the syntax of this model is pretty much straight forward for someone to be used, just outside the box. But a lot of hyperparameters need to be set in order for the Fitting to start which can be cumbersome as the number of features increases.
    \item The fitting of the model starts to take more time as number of features increases. Because as the number of features increases the splines used also increases \& more Splines takes up more training time. Hence, for larger models, the training time is very high.
    
\end{itemize}






==> GP_Sparsh.tex <==
\subsection{Genetic Programming (GP) Approaches}

When it comes to Machine Learning Algorithms in \textbf{Interpretable AI} then Genetic Algorithms (GA) also comes to our mind, due to it's much decipherable hyperparameters \& tuning parameter.

\noindent For Genetic Algorithm to be tested on the same set of Data as other Algorithms are tested on we employee the use of \textbf{Gplearn}, developed by Trevor Stephens.

\noindent As the code for Gplearn is Open-Source, hence it's code was altered in order to obtain various Parameters required to Analyze the interpretability of the Algorithm.

The Genetic Algorithms are based on the Darwin's Theory of Evolution of Species over a period of time. Like the Organisms are said to be evolve and adapt according to their environment and the conditions that they are subjected to, for their survival. Hence, the Genetic Algorithms also revolves around this concept only.

% Figure \ref{fig:values_truss represents values obtain for Truss problem.

\begin{figure}[hbtp]
    \centering
    \includegraphics[scale = 0.5 ]{GAfigures/GradientDescentClassicalMethod.png}
    \caption{Gradient Descent for Optimization. \Yashesh{Sparsh, is this our original figure?}\Sparsh{Yes}}
    \label{fig: Gradient Descent for optimization}
\end{figure}

We know that for an Optimization problem we do have traditional techniques to find the solution by \textbf{Gradient Descent} \& whilst keeping a \textbf{Learning Rate} for the Problem. In which we tend to move iteratively towards the Minima, by working through the Steepest Descent, on the Contours of the Function.

But on the other hand, with Genetic Algorithm, our approach to solve that problem would be as follows:-
\begin{enumerate}
    \item We would \textbf{initialize} our Programs (which are the proposed solution to problem), most likely randomly.
    
    \item After the initialization, we will be evaluating them, based on a \textbf{Fitness criteria} (it's choice can depend from problem-to-problem), a Fitness Function's value is to be \textbf{maximised} for a program of GA, eg:- the function's value. Therefore, from the Fitness Function we obtain the Fitness values of the Programs.
    
    \item Based on the Fitness values of the Genetic Programs \& some other criterias(or randomness) which could be introduced by us, we can
\end{enumerate}

\begin{figure}[hbtp]
    \centering
    \includegraphics[scale = 0.5]{GAfigures/GAflowchart.png}
    \caption{Working of Genetic Algorithm}
    \label{fig:Working of Genetic Algorithm}
\end{figure}

\subsubsection{Results On Datasets}
\begin{table*}[ht]
\centering
\caption{GP Results: Parsimony Coefficient (PC) = 0.01. Have the results for (PC = 0.001, 0.005).}
\label{tab:gp_results_old}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Sr. No.} & \textbf{Datasets}               &
\begin{tabular}{c}
    \textbf{\#Unique} \\
    \textbf{Features}
\end{tabular} & \begin{tabular}{c}
     \textbf{\#Constants}\\
     \textbf{AtTerminals}
\end{tabular}  & \begin{tabular}{c}
     \textbf{\#TotalFeatures}\\
     \textbf{AtTerminal}
\end{tabular} & \begin{tabular}{c}
     \textbf{\#Internal}\\
     \textbf{Nodes}
\end{tabular} & \begin{tabular}{c}
     \textbf{Training}\\
     \textbf{Accuracy}
\end{tabular} & \begin{tabular}{c}
     \textbf{Testing}\\
     \textbf{Accuracy}
\end{tabular}  \\ \hline
1                & DS1                             & 1.54 ± 0.5                    & 1.24 ± 0.52                     & 1.86 ± 1.07                            & 2.1 ± 1.54                   & 59.99 ± 8.41               & 64.63 ± 10.37             \\ \hline
2                & DS2                             & 2.0 ± 0.0                     & 0.0 ± 0.0                       & 3.0 ± 0.0                              & 2.0 ± 0.0                    & 95.24 ± 0.0                & 95.24 ± 0.0               \\ \hline
3                & DS3                             & 2.0 ± 0.0                     & 1.0 ± 0.97                      & 3.6 ± 1.41                             & 3.6 ± 2.08                   & 61.31 ± 9.95               & 61.87 ± 10.04             \\ \hline
4                & DS4                             & 0.78 ± 0.76                   & 1.26 ± 1.71                     & 2.02 ± 3.2                             & 2.28 ± 4.32                  & 50.69 ± 2.07               & 48.7 ± 2.86               \\ \hline
5                & Truss                           & 2.36 ± 0.56                   & 0.92 ± 1.08                     & 6.22 ± 4.2                             & 6.14 ± 4.26                  & 85.83 ± 9.51               & 82.98 ± 10.02             \\ \hline
6                & Welded Beam                     & 2.88 ± 0.69                   & 1.62 ± 1.54                     & 8.34 ± 4.57                            & 8.96 ± 4.72                  & 83.35 ± 12.62              & 83.58 ± 12.42             \\ \hline
7                & Cancer (10F) & 2.92 ± 1.1                    & 2.7 ± 1.87                      & 4.96 ± 2.25                            & 6.66 ± 2.02                  & 94.84 ± 4.47               & 93.17 ± 4.39              \\ \hline
8                & Cancer (30F) & 3.9 ± 0.84                    & 0.02 ± 0.14                     & 5.76 ± 1.71                            & 4.78 ± 1.72                  & 90.42 ± 5.9                & 90.33 ± 6.09              \\ \hline
9                & dtlz1\_3\_30                    & 1.96 ± 2.07                   & 0.44 ± 0.64                     & 2.34 ± 2.96                            & 1.78 ± 3.09                  & 63.37 ± 14.97              & 62.62 ± 14.42             \\ \hline
10               & dtlz1\_3\_500                   & 2.1 ± 0.91                    & 0.02 ± 0.14                     & 2.12 ± 0.94                            & 1.14 ± 0.9                   & 72.95 ± 8.57               & 72.37 ± 8.48              \\ \hline
11               & dtlz2\_3\_30                    & 1.36 ± 1.16                   & 0.4 ± 0.61                      & 1.78 ± 2.45                            & 1.18 ± 2.56                  & 65.57 ± 14.69              & 64.92 ± 14.19             \\ \hline
12               & dtlz2\_3\_500                   & 2.0 ± 0.61                    & 0.06 ± 0.24                     & 2.18 ± 1.76                            & 1.24 ± 1.73                  & 73.38 ± 9.32               & 72.77 ± 9.13              \\ \hline
\end{tabular}
\end{table*}

\noindent {\bf Advantages:}
\begin{itemize}
    \item The tree-based Genetic Programs are very much intuitive and explainable to non-technical people as well.
    \item The API of Gplearn is very straight-forward to be used, on any dataset.
    \item The API also offers very much flexibility, eg- to add some customized operator, fitness function etc.
    \item 
    
\end{itemize}

\noindent {\bf Disadvantages:}
\begin{itemize}
    \item Due to random state with no seed being used, the tree varies a lot in structure with repeated runs.
    \item Their many hyperparameters to be set for a run on a Dataset, though the default parameter values can be used.
    \item Redundancy in tree can also occur.
    
\end{itemize}


Here we will show some plots...
Figure \ref{fig:values_truss} represents values obtain for Truss problem.
\begin{figure}[hbtp]
    \centering
    \includegraphics[width = \linewidth]{figures/Values_dist_truss.jpeg}
    \caption{Truss Values. \Yashesh{Sparsh, You will then have to put the statistics on EoDF in the big summary table.}}
    \label{fig:values_truss}
\end{figure}


==> extra_tables.tex <==
\begin{table*}[hbt]
\caption{Benchmarking against datasets from different sources.}
    \label{tab:benchmarking_from_different_sources}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}\hline
        \textbf{Dataset} & 
        \begin{tabular}{c}
             \textbf{Training}\\
             \textbf{Accuracy}
        \end{tabular} & 
        \begin{tabular}{c}
             \textbf{Testing}\\
             \textbf{Accuracy}
        \end{tabular} & 
        \textbf{\# Rules} & 
        \begin{tabular}{c}
             \textbf{Average}\\
             \textbf{Rule Len.}
        \end{tabular} & 
        \begin{tabular}{c}
             \textbf{Total}\\
             \textbf{Rule Len.}
        \end{tabular} \\\hline
        \multicolumn{6}{|c|}{NLDT} \\\hline
        DS1-MATLAB & $ 99.66 \pm  0.69 $ & $ 98.87 \pm 1.81 $ &  $ 1.00 \pm 0.00 $ & $ 2.46 \pm 0.64 $ & $ 2.46 \pm 0.64 $ \\\hline
        DS1-MATLAB2 & $ 98.66 \pm  1.27 $ & $ 97.63 \pm 2.83 $ & $ 1.22 \pm 0.46 $ & $ 2.52 \pm 0.55 $ & $ 3.04 \pm 1.15 $ \\\hline

        DS1-SPARSH &  $ 98.66 \pm  1.27 $ & $ 97.63 \pm 2.83 $ & $ 1.22 \pm 0.46 $ & $ 2.52 \pm 0.55 $ & $ 3.04 \pm 1.15 $ \\\hline

        \multicolumn{6}{|c|}{NLDT} \\\hline
        DS2-MATLAB & $ 98.38 \pm  1.47 $ & $ 97.21 \pm 2.28 $ &  $ 1.00 \pm 0.45 $ & $ nan \pm nan $ & $ 2.70 \pm 1.32 $ \\\hline
        \multicolumn{6}{|c|}{NLDT} \\\hline
        DS3-MATLAB & $ 99.66 \pm  0.77 $ & $ 98.73 \pm 2.15 $ &  $ 1.08 \pm 0.39 $ & $ 2.34 \pm 0.68 $ & $ 2.50 \pm 1.00 $ \\\hline
        DS3-SPARSH & $ 98.64 \pm  0.95 $ & $ 97.00 \pm 2.69 $ & $ 1.32 \pm 0.58 $ & $ 2.38 \pm 0.62 $ & $ 3.10 \pm 1.39 $ \\\hline
    \end{tabular}
\end{table*}

==> random_template.tex <==

%...Template for the Summary of Results Table
PROB & 
\begin{tabular}{c}
  Accuracy \\ Complexity 
\end{tabular} & 
\begin{tabular}{c}
  NDLT \\ NLDT
\end{tabular} & 
\begin{tabular}{c}
  CART \\ CART 
\end{tabular} & 
\begin{tabular}{c}
  SVM \\ SVM 
\end{tabular} & 
\begin{tabular}{c}
  GAM \\ GAM 
\end{tabular} & 
\begin{tabular}{c}
  GP \\ GP
\end{tabular} \\\hline
